Mitigating Object Hallucinations in Large Vision-Language Models through Visual Contrastive Decoding

Large Vision-Language Models (LVLMs) have advanced considerably, intertwining visual recognition and language understanding to generate content that is not only coherent but also contextually attuned. Despite their success, LVLMs still suffer from the issue of object hallucinations, where models generate plausible yet incorrect outputs that include objects that do not exist in the images. To mitigate this issue, we introduce Visual Contrastive Decoding (VCD), a simple and training-free method that contrasts output distributions derived from original and distorted visual inputs. The proposed VCD effectively reduces the over-reliance on statistical bias and unimodal priors, two essential causes of object hallucinations. This adjustment ensures the generated content is closely grounded to visual inputs, resulting in contextually accurate outputs. Our experiments show that VCD, without either additional training or the usage of external tools, significantly mitigates the object hallucination issue across different LVLM families. Beyond mitigating object hallucinations, VCD also excels in general LVLM benchmarks, highlighting its wide-ranging applicability.

==> 03_invest.tex <==
\section{Investigating Object Hallucinations}
\label{sec:invest}

\input{figs/figure2}

\subsection{Statistical Bias \& Unimodal Priors in LVLMs}
% However, in cases where the training corpus of $\theta$ exhibits statistical bias (e.g., spurious correlations among objects) or input queries contain out-of-distribution knowledge with respect to $\theta$, we hypothesize that the model can struggle to effectively attend to $\boldsymbol{x}$\&$\boldsymbol{v}$ and overly rely on the prior knowledge encoded in $\theta$, which may be influenced by statistical bias residing in training corpus.
%\lx{Note: IMO, both statistical bias and language prior are learned biases but of different types (one from cross-modal pre-training and the other from text-based pre-training), so we better give more self-explanatory names to them}
%Sicong: IMO, biases are wrong embeded knowledge, while priors are general helpful knowledge but should not overshadow the real inputs.
% \lx{Note: for better understanding, shall we explicitly define these two concepts at the beginning of this passage?}
% Despite the success of LVLMs, challenges arise when their training corpus is marred by statistical bias (e.g., spurious correlations among objects) or when the model excessively relies on unimodal priors to generate the response\lx{MARK}. We hypothesize that under these conditions, the model may encounter difficulties in effectively attending to both textual and visual inputs. Instead, it may exhibit an over-reliance on unimodal priors and statistical biases encoded in during pre-training\lx{Note: this paragraph is still not good, need to rewrite}.
In the realm of LVLMs, previous works find that object hallucinations primarily arise from two factors:  (1) statistical biases in training data and (2) over-reliance on unimodal priors~\cite{agarwal2020towards,agrawal2016analyzing,goyal2017making,li2023evaluating,yan2023overcoming,zhibo2023overcoming,han2022visual,wu2022overcoming,gupta2022swapmix,niu2021counterfactual}. 
%These biases, often presented as erroneous object correlations, leading to the generation of contextually misaligned responses\lx{$\Rightarrow$ Statistical biases are typically presented as frequent but superficial object correlations. These biases often lead to the generation of undesirable objects in the responses}
% \lx{Note: can move these two sentences right after the description of statistical biases in the 2nd paragraph}. 
% This issue is further compounded by an overly dependence on unimodal, especially language, priors ingrained during the integrated LLMs' pretraining phase, compelling the models to favor textual patterns over actual visual inputs. Together, these factors significantly compromise the models' ability to accurately integrate and interpret multimodal information, making hallucinations a prominent challenge in LVLMs\lx{Note: The last two sentences can be removed}.
%Statistical biases within the training datasets of LVLMs present a significant challenge, often resulting in the emergence of object hallucination during the inference stage\lx{remove this sentence}\lx{Note: no need to say the statistical biases will lead to object hallucination here}. 
Statistical biases within training datasets of LVLMs typically result from imbalanced data distributions and the over-representation of specific objects or patterns~\cite{agarwal2020towards,agrawal2016analyzing,goyal2017making,li2023evaluating}.
%, which are typically presented as frequent but superficial object correlations\lx{$\Rightarrow$ and over-representation of co-occurrence patterns, and they are generally presented as frequent but superficial object correlations.} 
Such biases are typically presented as frequent but superficial object correlations, leading to the generation of contextually misaligned objects in the responses\lx{MARK}.
% Consequently, spurious correlations between visual and textual elements become embedded within the model, leading to unfounded associations and predictions\lx{$\Rightarrow$ Such spurious correlations between visual and textual elements will lead to the generation of undesirable objects in the responses}.
For example, if a dataset consistently associates a particular object (e.g., \textit{dining table}) with specific contexts (e.g., \textit{chair}) or attributes, the trained model is likely to generate descriptions incorporating this object, even in instances where the visual input does not include such associations. 
%This inclination towards relying on biased correlations undermines the model's capacity to generate contextually accurate and relevant content, particularly in diverse and dynamic real-world scenarios.

The over-reliance on unimodal priors is another pervasive issue complicating the efficacy of LVLMs~\cite{yan2023overcoming,zhibo2023overcoming,han2022visual,wu2022overcoming,gupta2022swapmix,niu2021counterfactual}. This phenomenon is characterized by the models' inclination to depend solely on either textual or visual data during the inference process. 
%Such a dependency emerges as a consequence of the models' training dynamics, where biases inherent in the training data manifest as an imbalanced utilization of the input modalities. 
This imbalance is particularly evident when LVLMs have to handle complex or ambiguous inputs. 
%In these situations, models tend to default to the more dominant modality, as conditioned by their training data. This dominant modality often overshadows the complementary data type, leading to outputs that, while potentially coherent, may lack contextual accuracy and depth. 
% \textbf{(talk more about language priors in LLMs)}
Specifically, LVLMs often adopt language priors from their integrated foundational Large Language Models (LLMs). These priors are typically the knowledge and patterns learned from massive textual pre-training~\cite{brown2020language,bender2021dangers}. Although language priors are generally helpful in commonsense reasoning, they can also overshadow fresh visual inputs, especially when such data is uncertain or noisy\lx{MARK}
% For instance, consider an image of a rarely-seen bird perched on a "\textit{computer keyboard}". When this image is fed into an LVLM along with a partial caption like "\textit{The bird is on the...}", given the dominance of language priors from LLMs, the model might be inclined to complete the sentence as "\textit{The bird is on the tree branch}" rather than "\textit{The bird is on the computer keyboard.}" This is because, in most textual data, birds are more commonly associated with trees than with computer keyboards. The model defaults to the more frequently seen scenario in its textual training, even if it mismatches the visual data provided. This exemplifies the LVLM's over-reliance on its ingrained language priors at the expense of current visual information.
For example, regardless of the actual color of the banana depicted in a given image, a model overly reliant on language priors might consistently respond with ``\textit{yellow}'' to the query ``\textit{What is the color of the banana in this image?}'', highlighting its tendency to prioritize embedded textual knowledge over the specific visual information provided.
%The models’ outputs, in such cases, reflect a skewed integration of visual and textual information, resulting in responses that are not fully representative of the input data’s multimodal nature.

\input{figs/bias}
\subsection{Visual Uncertainty Induces
More Object Hallucinations}
The fidelity of visual input is pivotal for LVLMs to accurately encode visual features and generate outputs faithfully. Yet, the introduction of uncertainty in visual inputs can tilt the equilibrium. This section delves into a comprehensive analysis aimed at validating the assumption that increased visual uncertainty can exacerbate the object hallucination issues in LVLMs' generative processes.

\paragraph{Introduction of Visual Uncertainty}
%\paragraph{Image-Level Distortion}
In the most elementary form of introducing visual uncertainty, a Gaussian noise mask is applied to the original image. This blanket distortion, although straightforward, provides an initial benchmark to estimate the baseline effects of visual uncertainty on model outputs. Following the forward diffusion process in image generation~\cite{ho2020denoising}, the distorted image is modeled as follows:
\begin{equation}
\label{eq:1}
\begin{aligned}
&q\left({v}_t \mid {v}_{t-1}\right)=\mathcal{N}\left({v}_t ; \sqrt{1-\gamma} {v}_{t-1}, \gamma \mathbf{I}\right) \\
&q\left({v}_{T} \mid {v}_0\right)=\prod_{t=1}^T q\left({v}_t \mid {v}_{t-1}\right),
\end{aligned}
\end{equation}
where $v_0$ is an original image, and we add a small amount of Gaussian noise to the image in $T$ steps, producing a sequence of distorted images $v_1,\dots,v_T$. The original image $v_0$ gradually loses its distinguishable features as step $t$ becomes larger, where the amount of noise added in each step is controlled by $\gamma$. Eventually, when $T \rightarrow \infty$, $v_T$ is equivalent to an isotropic Gaussian distribution\footnote{While this study employs a basic Gaussian noise approach, more fine-grained techniques, like object-level blurring, hold the potential for improved outcomes. Exploring such distortions is considered a direction for future research.}. 

\subsubsection{Visual Uncertainty Amplifies Language Priors}

Figure~\ref{fig: language priors} provides a case to show how visual distortion affects the predictions of LVLMs. As can be seen, given an image featuring a black banana among other colorful fruits, LVLMs favor more conventional banana colors—such as "\textit{yellow}" and "\textit{green}", with increasing visual uncertainty. The ground-truth color "\textit{black}" diminishes in probability as the distortion escalates, making LVLMs over-reliant on the language priors from LLM pre-training that typically associate bananas with being yellow or green. This tendency, which shows that visual uncertainty can compel LVLMs to overlook visual evidence and overly exploit language priors for decision-making, is not entirely unexpected.
%This amplification in the reliance on language priors is not entirely unexpected. 
LLMs are designed to predict next-word probabilities based on vast textual corpora. When confronted with ambiguous or uncertain visual stimuli, an LVLM might default to these robust, text-based predictions as a ``safety net''. These priors, while generally useful, can introduce biases or assumptions inconsistent with the actual visual content, particularly when the visual input lacks clarity. 
%Thus, in scenarios where visual uncertainty is high, the LVLMs might inadvertently prioritize their embedded language priors inherited from LLMs, elevating the risk of hallucinations.
% \textbf{(explain about uncertainty in visual inputs will amplify reliance on language priors in LLMs which is quite straightforward)}
% An assumption central to our study is that this phenomenon of heightened hallucination arises as a direct consequence of the ambiguity introduced in the visual inputs.
%当visual被distorted了，over-reliance on language prior in LLM很直接，这儿主要是证明statistical bias是否也更严重了。
% \textbf{(Verify assumptions that uncertainty in visual inputs also amplify statistical bias from two experiments)}
% \textbf{(1. if LVLMs hallucinate frequent objects more with distorted visual inputs; 2. if LVLMs are more prone to hallucinate objects that frequently co-occur with gt objects in the image)}
% To verify this assumption, we embarked on a systematic experimental investigation.
\subsubsection{Visual Uncertainty Amplifies Statistical Bias}
%Prior works~\cite{li2023evaluating,liu2023mitigating} have pointed out that statistical biases, such as frequent visual co-occurrence patterns within pretraining datasets, are significant contributors to object hallucinations in LVLMs. 
Here we posit a supplementary hypothesis: visual uncertainty not only bolsters the model's dependence on language priors but may also amplify these statistical biases from pretraining. To examine this hypothesis more rigorously, we designed two targeted experiments to verify: (1) if LVLMs hallucinate frequent objects more with distorted visual inputs; (2) if LVLMs are more prone to hallucinate objects that frequently co-occur with ground truth objects in the image with distorted visual inputs.
% Previous studies~\cite{li2023evaluating,liu2023mitigating} have verified that statistical biases such as object frequencies and co-occurrences in pertaining datasets are one of the major causes of the object hallucination issue.
% However, another assumption underpins our exploration: not only does visual uncertainty increase the model's reliance on language priors, but it might also accentuate the statistical biases ingrained during the model's training. To examine this hypothesis more rigorously, we designed two targeted experiments to verify: (1) if LVLMs hallucinate frequent objects more with distorted visual inputs; (2) if LVLMs are more prone to hallucinate objects that frequently co-occur with ground truth objects in the image with distorted visual inputs.


\paragraph{Effect of Visual Uncertainty on Frequent Objects}
The construction of most visual instruction datasets is predominantly based on MSCOCO~\cite{lin2014microsoft}, which inherently suffers from an unbalanced object distribution. %Specifically, a minority of frequently appearing objects dominate the dataset. 
As LVLMs are fine-tuned on such data, they may inherit a predisposition to generate descriptions emphasizing, or even hallucinating, these prevalent objects from MSCOCO. 
%Given that we have access to ground-truth object annotations within MSCOCO, we sought empirical clarity on this matter. 
%A bar chart was formulated to elucidate the relationship between the three top-frequent objects in MSCOCO and the frequency of their hallucinations in its validation set. 
%This visualization offers a quantifiable perspective on how the prevalence of objects in the training dataset might influence a model's likelihood of hallucinating them, particularly under conditions of visual uncertainty.
As depicted in the left subfigure of Figure~\ref{fig:bias}, the correlation between frequent objects in MSCOCO and their propensity to be hallucinated in the validation set is evident. The chart showcases that objects with a higher occurrence rate in the dataset are, unsurprisingly, more likely to be hallucinated by LVLMs under distorted visual scenarios. 
%This observation underscores the model's vulnerability to the biases present in the training data, especially when presented with ambiguous visual cues. 
% Such a trend suggests that visual uncertainty does not just amplify the reliance on language priors but also accentuates the inherent statistical biases of the training data.

\paragraph{Effect of Visual Uncertainty on Co-occurring Objects}
To further probe the implications of visual uncertainty, we also evaluate the impact on frequently co-occurring object groups. Using the "\textit{dining table}" as a representative object, we analyzed its frequent co-occurrences in the MSCOCO dataset. In the right subfigure of Figure~\ref{fig:bias}, we chart the three objects that often appear alongside the "\textit{dining table}". The data reveals a notable pattern: objects with higher co-occurrence rates with the "dining table" are also more frequently hallucinated by LVLMs when presented with distorted visual inputs. 
This further validates our hypothesis that visual uncertainty exacerbates the model's tendency to lean on ingrained statistical biases.

% In summation, our examination underscores that visual uncertainty not only amplifies the reliance on language priors but also accentuates the LVLM's inclination towards statistical biases inherent in training datasets. The phenomena of over-generating frequent objects and the heightened susceptibility to hallucinate co-occurring objects with uncertain visuals underscore this observation. 
% Building on our findings, it's evident that the output distributions from LVLMs, when faced with distorted visual inputs, are skewed towards hallucinations. This insight provides a pivotal motivation for our Visual Contrastive Decoding (VCD) methodology. 
% By identifying those language priors and statistical bias amplified by visual uncertainty, VCD aims to effectively counteract or contradict these consequent hallucinations. The underlying principle is straightforward: VCD contrasts output distributions from both original and distorted visual inputs. By highlighting differences between these distributions, VCD effectively pinpoints and mitigates hallucinations, ensuring model outputs that are more anchored to the immediate visual context.
In summation, our study reveals that visual uncertainty not only amplifies reliance on language priors but also heightens LVLMs' tendencies towards statistical biases present in training datasets. These tendencies manifest as over-generation of frequent objects and an increased likelihood of hallucinating co-occurring objects. %Notably, when LVLMs encounter distorted visuals, their output distributions tend to favor hallucinations. 
This observation forms the foundation for our Visual Contrastive Decoding (VCD) approach, which aims to counterbalance these biases by contrasting outputs from original and distorted visual inputs. 
%By discerning these differences, VCD effectively reduces hallucinations, ensuring outputs that align closely with the visual context.


==> figs/case_small.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=1\linewidth]{figs/case_small_.pdf}
    \caption{Examples from LLaVA-Bench of our proposed VCD for hallucination corrections. Hallucinated objects from LVLM's regular decoding are highlighted in \color{red}{red}.}
    \label{fig:case study}
    \vspace{-0.4cm}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/GPT4_evaluator_case.tex <==
% GPT4_prompt
